A reconstructed discontinuous approximation for distributed elliptic control problems

In this paper, we present and analyze an interior penalty discontinuous Galerkin method for the distributed elliptic optimal control problems. It is based on a reconstructed discontinuous approximation which admits arbitrarily high-order approximation space with only one unknown per element. Applying this method, we develop a proper discretization scheme that approximates the state and adjoint variables in the approximation space. Our main contributions are twofold: (1) the derivation of both a priori and a posteriori error estimates of the $L^2$-norm and the energy norms, and (2) the implementation of an efficiently solvable discrete system, which is solved via a linearly convergent projected gradient descent method. Numerical experiments are provided to verify the convergence order in a priori error estimate and the efficiency of a posteriori error estimate.

==> numerical_corex.tex <==
\section{Numerical Results}
It should be noted that the approximate system $\eqref{eq10}$ 
can not be solved directly.
So we will first introduce a projected gradient descent 
method to solve $\eqref{eq10}$ iteratively in Section 5.1. In 
Section 5.2, we provide some numerical examples to validate 
the derivation in the previous sections, including a priori and a 
posteriori error estimates. In the case that the control variable has 
a smooth data, we can build another approximation to $\eqref{eq27}$
without $\mathcal{T}^h_u$, which 
means that we do not discretize the control variable. 
The proposed approximation serves to significantly improve 
computational efficiency and offers the advantage of reduced 
memory consumption.

\subsection{Practical Algorithm}
Take $u_{h0}\in U_{adh}$ as an  
initial guess to $u_h^*$ , we can then obtain a sequence \{($u_{hn},y_
{hn}^m,p_{hn}^m)\}_{n=0} ^\infty$ by the following algorithm.
\begin{equation}\label{eq5.1}
\left\{
\begin{aligned}
&a_{h,\theta}(y_{hn}^{m},w_{h}^m)=l_{h,\theta}[f+Bu_{hn}
,\phi](w_{h}^m),\quad\forall w_{h}^m\in V_h^m,\\
&a_{h,\theta}(q_h^m,p_{hn}^{m})=l_{h,\theta}[g^\prime(y_{hn}^
{m}),0](q_h^m),\quad\forall q_h^m\in V_h^m,\\
&u_{h \mkern+1mu n \mkern-2mu+\mkern-2mu 1}=Pr_{U_{adh}}
(u_{hn}-\rho_n(j'(u_{hn})+B^*p_{hn}^m)),
\end{aligned}
\right.
\end{equation}
where $Pr_{U_{adh}}:U\rightarrow U_{adh}$ is the projection
 operator and $\rho_n>0,\forall n\in \mathbb{N}.$

\begin{thm}\label{thm6}
Let $(u_h^*,y_h^{m*},p_h^{m*})$ satisfy $\eqref{eq10}$, $\{(u_{hn},
y_{hn}^m,p_{hn}^m)\}_{n=0}^\infty$ be the sequence generated by 
$\eqref{eq5.1}$. If Assumption $\eqref{ass1}$,$\eqref{ass2}$ 
hold, we can properly  
choose $\{\rho_n\}_{n=0}^\infty$ such that there exist constants
$0<\eta<1,\lambda=\lambda(\eta)>0,$ satisfy
\begin{equation*}
\begin{aligned}
&\|u_{hn}-u_h^*\|_{L^2}+\lambda\interleave y_{hn}
^m-y_h^{m*}\interleave_{\mathrm{DG}}+\lambda\interleave p_{n}^m-p_h^{m*}\interleave_{\mathrm{DG}}\\
\leq& \eta^n(\|u_{h0}-u_h^*\|_{L^2}+\lambda\interleave y_{h0}^m-y_h^{m*}\interleave_{\mathrm{DG}}+\lambda\interleave
 p_{h0}^m-p_h^{m*}\interleave_{\mathrm{DG}}).
\end{aligned}
\end{equation*}
In fact, we can show that $(u_{hn},y_{hn}^m,p_
{hn}^m)$ converges to $(u_{h}^*,y_{h}^{m*},p_{h}^{m*})$ linearly. 
\end{thm}

\begin{proof}
From now on, we omit the superscript $*$. We have
\begin{equation*}
\begin{aligned}
\|u_{h\mkern+1mu n\mkern-2mu+\mkern-2mu 1}-u_h\|_{L^2}^2=
&\|Pr_{U_{adh}}(u_{hn}-\rho_n(j'(u_{hn})+B^*p_{hn}^m))\\
&-Pr_{U_{adh}}(u_{h}-\rho_n(j'(
u_{h})+B^*p_{h}^m))\|_{L^2}^2\\
\leq&\|u_{hn}-u_{h}-\rho_n(j'(u_{hn})-j'(
u_{h})+B^*p_{hn}^m-B^*p_{h}^m)\|_{L^2}^2\\
=&\|u_{hn}-u_{h}\|_{L^2}^2+\rho_n^2\|j'(u_{hn})-j'(
u_{h})+B^*p_{hn}^m-B^*p_{h}^m\|_{L^2}^2\\
&-2\rho_n(u_{hn}-u_h,j'(u_{hn})-j'(u_h)+B^*p_{hn}^m-B^*p_h^m)\\
\leq&(1-2\alpha\rho_n+C\rho_n^2)\|u_{hn}-u_{h}\|_{L^2}^2+
C\rho_n^2\|p_{hn}^m-p_h^m\|_{L^2}^2\\
&-2\rho_n(u_{hn}-u_h,B^*p_{hn}^m-B^*p_h^m).
\end{aligned}
\end{equation*} 

From $\eqref{eq10},\eqref{eq5.1}$ we have
\begin{equation}\label{eq5.2}
\begin{aligned}
&a_{h,\theta}(y_{hn}^m-y_h^m,w_h^m)=(B(u_{hn}-u_h),w_h^m),\quad\forall w_h^m
\in V_h^m,\\
&a_{h,\theta}(q_h^m,p_{hn}^m-p_h^m)=(g^\p(y_{hn}^m)-g^\p(y_h^m),q_h^m),\quad
\forall q_h^m\in V_h^m.
\end{aligned}
\end{equation}
Let $w_h^m=p_{hn}^m-p_h^m,q_{hn}^m=y_{hn}^m-y_h^m.$ Then
\begin{equation*}
\begin{aligned}
&(u_{hn}-u_h,B^*p_{hn}^m-B^*p_h^m)=(B(u_{hn}-u_h),p_{hn}^m-
p_h^m)\\
=&(g^\p(y_{hn}^m))-g^\p(y_h^m),y_{hn}^m-y_h^m)\geq
\beta\|y_{hn}^m-y_h^m\|_{L^2}^2\geq0.
\end{aligned}
\end{equation*}
Let $w_h^m=y_{hn}^m-y_h^m,q_{hn}^m=p_{hn}^m-p_h^m.$ By the 
stability of $a_{h,\theta}$ on $(V_h^m,\interleave\cdot\interleave
_{\mathrm{DG}})$ and $\eqref{eqb}$, we know that
\[\interleave y_{hn}^m-y_h^m\interleave_{\mathrm{DG}}\leq C
\|u_{hn}-u_h\|_{L^2},
\quad\interleave p_{hn}^m-p_h^m\interleave _{\mathrm{DG}}\leq C
\|y_{hn}^m-y_h^m\|_{L^2}.\]

Consequently,
\[\|u_{h \mkern+1mu n \mkern-2mu+\mkern-2mu 1}-u_h\|_{L^2}^2
\leq(1-2\alpha\rho_n+C\rho_n^2)\|u_{hn}-u_h\|_{L^2}^2\leq
\delta^2\|u_{hn}-u_h\|_{L^2}^2,\]
where $\rho_n$ satisfies $0\leq1-2\alpha\rho_n+C\rho
_n^2\leq\delta^2<1,\forall n\in\mathbb{N}.$ 
Choose $C'$ such that
\[\interleave y_{h \mkern+1mu n \mkern-2mu+\mkern-2mu 1}^m-y_h^m\interleave_{\mathrm{DG}}+\interleave p_{h \mkern
+1mu n \mkern-2mu+\mkern-2mu 1}^m-p_h
^m\interleave_{\mathrm{DG}}\leq C'\|u_{h \mkern+1mu n \mkern
-2mu+\mkern-2mu 1}-u_h\|_{L^2},\]
and $\lambda=(1-\delta)/(2C'\delta)$. It can be verified that
\begin{equation*}
\begin{aligned}
&\|u_{h \mkern+1mu n \mkern-2mu+\mkern-2mu 1}-u_h\|_{L^2}
+\lambda\interleave y_{h \mkern+1mu n \mkern-2mu+\mkern-2mu 1}^m-y_h^m\interleave_{\mathrm{DG}}+\lambda\interleave p_{h 
\mkern+1mu n \mkern-2mu+\mkern-2mu 1}^m-p_h
^m\interleave_{\mathrm{DG}}\\
\leq& \frac{\delta+1}{2}(\|u_{hn}-u_h\|_{L^2}+\lambda\interleave y_{hn}^m-y_h^m\interleave_{\mathrm{DG}}+\lambda
\interleave p_{hn}^m-p_h^m\interleave_{\mathrm{DG}}),
\end{aligned}
\end{equation*}
which means the linear convergence rate. To complete the proof, 
we only need to take $\eta=(\delta+1)/2$.
\end{proof}

%For simplicity,  we introduce two notations
%$$[\ \cdot\ ]_{\mathrm{DG}}:=\|u^*-u_h^*\|_{L^2}
%\interleave y^*-y_h^{m*}\interleave_{\mathrm{DG}}+\interleave p^*-p_h^{m*}\interleave_{\mathrm{DG}},$$
%$$[\ \cdot\ ]_{L^2}:=\|u^*-u_h^*\|_{L^2}+
%\| y^*-y_h^{m*}\|_{L^2}+\| p^*-p_h^{m*}\|_{L^2}.$$

\subsection{Numerical Examples}
\mbox{}\\
\noindent\textbf{Examples for Convergence Order.}
We will use some examples to verify the convergance order 
proved in Theorem $\eqref{thm2}$ and Lemma $\eqref{lem2}.$

\noindent\textbf{Example 1.} Take $\Omega_u=\Omega=(0,1)^2,
B=\mathrm{Id}.$
\begin{equation*}
\begin{aligned}
&\min_{u\in L^2(\Omega_u)}\frac{1}{2}\|y-y_d\|_
{L^2}^2+\frac{1}{2}\|u-u_d\|_{L^2}^2,
&\\s.t.\ &-\Delta y=f+u,\quad y|_{\partial\Omega}=y_d|_
{\partial\Omega},\\
& u\geq 0,\quad \mathrm{a.e.\ in}\ \Omega_u.
\end{aligned}
\end{equation*}
where
\begin{equation*}
\begin{aligned}
&y_d=0,\quad u_d=1-\mathrm{sin}\frac{\pi x_1}{2}-\mathrm{sin}
\frac{\pi x_2}{2},\\
&p=\mathrm{sin} (\pi x_1) \mathrm{sin} (\pi x_2),\quad f=4\pi^4
p-\mathrm{max}\{u_d-p,0\}.
\end{aligned}
\end{equation*}
The exact solution
\begin{equation*}
y^*=2\pi^2p+y_d,\quad u^*=\mathrm{max}\{u_d-p,0\},\quad 
p^*=p.
\end{equation*}

\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&6.499e-2&3.749e-2&1.913e-2&9.660e-3\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&3.070e1&1.356e1&6.091&2.835\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&1.568&7.041e-1&3.143e-1&1.447e-1\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&6.637e-2&3.752e-2&1.914e-2&9.660e-3\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&2.314e1&1.015e1&4.475&2.069\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&1.212&5.177e-1&2.269e-1&1.048e-1\\
\cline{2-7}
&\multirow{3}{*}{$4h^2\ \, $}&$\|u-u_h\|_{L^2}$&6.637e-2&1.929e-2&4.896e-3&1.225e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&8.103e-1&2.018e-1&4.542e-2&1.069e-2\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&5.917e-2&1.658e-2&3.886e-3&9.823e-4\\
\hline
\end{tabular}

\caption{Table 1 Numerical results of Example 1 for $m=1$.}
\end{table}

\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&6.643e-2&1.932e-2&4.925e-3&1.244e-3\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&1.109e1&2.643&6.584e-1&1.687e-1\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&6.040e-1&2.649e-1&7.405e-2&1.981e-2\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&6.530e-2&1.916e-2&4.854e-3&1.216e-3\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&8.853&1.971&4.732e-1&1.181e-1\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&4.877e-1&1.034e-1&2.426e-2&6.007e-3\\
\cline{2-7}
&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.556e-2&9.685e-3&1.221e-3&1.523e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&5.608e-1&4.872e-2&4.884e-3&5.527e-4\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&4.868e-2&3.632e-3&3.136e-4&3.098e-5\\
\hline
\end{tabular}

\caption{Numerical results of Example 1 for $m=2$.}
\end{table}

\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.730e-2&9.662e-3&1.217e-3&1.523e-4\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&3.244&4.010e-1&4.418e-2&4.619e-3\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&1.688e-1&2.122e-2&2.290e-3&2.361e-4\\
\hline
\multirow{3}{*}{-1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.684e-2&9.663e-3&1.217e-3&1.523e-4\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&2.914&4.215e-1&4.643e-2&5.365e-3\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&1.518e-1&2.097e-2&2.353e-3&2.718e-4\\
\hline
\end{tabular}

\caption{Numerical results of Example 1 for $m=3$.}
\end{table}

Recall that $R_h$ is the recovery operator defined in $\eqref{recover}$. 
We compute the error and convergence order of $\|u^*-R_hu_h^*
\|_{L^2}.$ 

\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l|l}
\hline
$\theta$&$m$&1/4&1/8&1/16&1/32&1/64&1/128\\
\hline\multirow{2}{*}{1}&1&8.528e-2&2.856e-2&1.102e-2&3.922e-3&1.371e-3&4.782e-4\\
\cline{2-8}
&2&6.175e-2&2.682e-2&1.035e-2&3.735e-3&1.327e-3&4.699e-4\\
\cline{1-1}\cline{2-8}
\multirow{1}{*}{-1}&1&6.198e-2&2.770e-2&1.074e-2&3.841e-3&1.351e-3&4.747e-4\\
\hline
\end{tabular}
\caption{Super-convergence results of Example 1.}
\end{table}

\noindent\textbf{Example 2.} Take $\Omega_u=\Omega=(0,1)^2,
B=\mathrm{Id}.$
\begin{equation*}
\begin{aligned}
&\min_{u\in L^2(\Omega_u)}\frac{1}{2}\|y-y_d\|_
{L^2}^2+\frac{1}{2}\|u-u_d\|_{L^2}^2,
&\\s.t.\ &-\nabla \cdot(A\nabla y) =f+u,\quad y|_{\partial\Omega}
=y_0|_{\partial\Omega},\\
& u\geq 0,\quad \mathrm{a.e.\ in}\ \Omega_u.
\end{aligned}
\end{equation*}
where
\begin{equation*}
\begin{aligned}
&A=\begin{bmatrix}
(x+1)^2&0\\
0&(y+1)^2
\end{bmatrix}
,\quad u_d=1-\frac23x_1-\frac23x_2,\\
&p=8x_1x_2(1-x_1)(1-x_2),\quad 
y_0=-\nabla \cdot(A\nabla p),\\
&f=-\nabla\cdot(A\nabla y_0)-\mathrm{max}\{u_d-p,0\},\quad
y_d=0.
\end{aligned}
\end{equation*}
The exact solution
\begin{equation*}
y^*=y_0,\quad u^*=\mathrm{max}\{u_d-p,0\},\quad 
p^*=p.
\end{equation*}
\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&7.393e-2&3.061e-2&1.437e-2&7.053e-3\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&2.578e1&1.178e1&5.275&2.429\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&8.059e-1&3.668e-1&1.673e-1&7.770e-2\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&8.684e-2&3.313e-2&1.472e-2&7.090e-3\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&2.587e1&1.188e1&5.283&2.426\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&8.876e-1&3.794e-1&1.701e-1&7.809e-2\\
\cline{2-7}
&\multirow{3}{*}{$4h^2\ \, $}&$\|u-u_h\|_{L^2}$&8.684e-2&2.290e-2&5.774e-3&1.368e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&1.164&3.607e-1&9.649e-2&2.388e-2\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&7.001e-2&1.824e-2&4.592e-3&1.050e-3\\
\hline
\end{tabular}
\caption{Numerical results of Example 2 for $m=1$.}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&5.679e-2&1.405e-2&3.507e-3&8.770e-4\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&7.684&1.339&2.889e-1&6.394e-2\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&3.577e-1&6.315e-2&1.253e-2&2.647e-3\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&5.821e-2&1.406e-2&3.510e-3&8.771e-4\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&8.314&1.458&2.925e-1&6.177e-2\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&3.993e-1&6.767e-2&1.371e-2&2.920e-3\\
\cline{2-7}
&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&5.821e-2&7.103e-3&8.848e-4&1.106e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&2.448e-1&2.695e-2&2.731e-3&2.947e-4\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&2.078e-2&1.140e-3&1.175e-4&1.493e-5\\
\hline
\end{tabular}
\caption{Numerical results of Example 2 for $m=2$.}
\end{table}
\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&5.511e-2&7.014e-3&8.770e-4&1.089e-4\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&1.361&9.444e-2&8.587e-3&9.587e-4\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&1.114e-1&7.828e-3&7.156e-4&7.884e-4\\
\hline
\multirow{3}{*}{-1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&5.503e-2&7.016e-3&8.770e-4&1.096e-4\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&1.506&1.023e-1&8.952e-3&9.667e-4\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&1.216e-1&8.484e-3&7.456e-4&8.055e-5\\
\hline
\end{tabular}
\caption{Numerical results of Example 2 for $m=3$.}
\end{table}

\noindent\textbf{Example 3.} Take $\Omega_u=\Omega=(0,1)^2,
B=\ds\frac{1}{2}\mathrm{Id}.$
\begin{equation*}
\begin{aligned}
&\min_{u\in L^3(\Omega_u)}\frac{1}{2}\|y-y_d\|_{L^2}^2+
\frac{1}{2}\|u-u_d\|_{L^2}^2+\frac{4}{3}\|u-u_d\|_{L^3}^3,
&\\s.t.\ &-\Delta y=f+\frac{1}{2}u,\quad y|_{\partial\Omega}=y_d|_
{\partial\Omega},\\
& 0\leq u\leq 1,\quad \mathrm{a.e.\ in}\ \Omega_u.
\end{aligned}
\end{equation*}
where
\begin{equation*}
\begin{aligned}
&u_d=\frac{3}{2}-x_1- x_2,\quad p=\mathrm{sin} (\pi x_1) \mathrm
{sin} (\pi x_2),\\
&y_d=0,\quad f=4
\pi^4p-\frac{1}{2}Pr_{[0,1]}(u_d-s(p)).
\end{aligned}
\end{equation*}
The exact solution
\begin{equation*}
y^*=2\pi^2p+y_d,\quad u^*=Pr_{[0,1]}(u_d-s(p)),\quad 
p^*=p,
\end{equation*}
where $s(p)$ is an implicit function satisfies \[s(p)+4
s(p)^2\mathrm{sgn}(s(p))=\frac{1}{2}p,\]
and $Pr_{[0,1]}(s):=\min\{\max\{s,0\},1\}.$
\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&1.109e-1&4.678e-2&1.887e-2&8.599e-3\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&2.967e1&1.455e1&6.578&2.950\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&1.803&8.943e-1&3.675e-1&1.522e-1\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&6.836e-2&3.340e-2&1.666e-2&8.338e-3\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&2.314e1&1.015e1&4.475&2.069\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&1.212&5.177e-1&2.269e-1&1.048e-1\\
\cline{2-7}
&\multirow{3}{*}{$4h^2\ \, $}&$\|u-u_h\|_{L^2}$&6.836e-2&1.697e-2&4.242e-3&1.059e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&8.101e-1&2.017e-1&4.540e-2&1.068e-2\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&5.915e-2&1.658e-2&3.885e-3&9.281e-4\\
\hline
\end{tabular}
\caption{Numerical results of Example 3 for $m=1$.}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&7.029e-2&1.697e-2&4.498e-3&1.135e-3\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&1.230e1&2.643&6.688e-1&1.739e-1\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&6.825e-1&1.450e-1&4.267e-2&1.183e-2\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&6.830e-2&1.665e-2&4.172e-3&1.043e-3\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&8.852&1.971&4.732e-1&1.182e-1\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&4.876e-1&1.034e-1&2.426e-2&6.007e-3\\
\cline{2-7}
&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.830e-2&8.364e-3&1.046e-3&1.305e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&5.605e-1&4.871e-2&4.883e-3&5.527e-4\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&4.866e-2&3.632e-3&3.135e-4&3.098e-5\\
\hline
\end{tabular}
\caption{Numerical results of Example 3 for $m=2$.}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.693e-2&8.333e-3&1.044e-3&1.305e-4\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&3.572&4.663e-1&5.377e-2&6.240e-3\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&1.836e-1&2.383e-2&2.733e-3&3.165e-4\\
\hline
\multirow{3}{*}{-1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.532e-2&8.344e-3&1.044e-3&1.305e-4\\
\cline{3-7}
&&$\interleave y-y_h^m\interleave_{\mathrm{DG}}$&2.914&4.125e-1&4.643e-2&5.365e-3\\
\cline{3-7}
&&$\interleave p-p_h^m\interleave_{\mathrm{DG}}$&1.518e-1&2.097e-2&2.353e-3&2.718e-4\\
\hline
\end{tabular}
\caption{Numerical results of Example 3 for $m=3$.}
\end{table}

Now we compute the error and convergence order of $\|u^*-R_hu_h^*
\|_{L^2}.$ 
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l|l}
\hline
$\theta$&$m$&1/4&1/8&1/16&1/32&1/64&1/128\\
\hline\multirow{2}{*}{1}&1&1.028e-1&3.572e-2&1.044e-2&2.968e-3&8.201e-4&2.549e-4\\
\cline{2-8}
&2&5.784e-2&1.328e-2&4.610e-3&1.629e-3&5.804e-4&2.275e-4\\
\cline{1-1}\cline{2-8}
\multirow{1}{*}{-1}&1&5.201e-2&1.600e-2&5.203e-3&1.752e-3&6.172e-4&2.122e-4\\
\hline
\end{tabular}
\caption{Super-convergence results of Example 3.}
\end{table}

\noindent\textbf{Smooth Example.}
Notice that in Theorem $\eqref{thm2}$ and Lemma $\eqref{lem2}$, the order 
of $h_u$ is rather small compared to $h$, which leads to more refinement on 
$\mathcal{T}^h_u$. In order to optimize computional efficiency and minimize
memory cost, we can calculate $u$ without discretization and eliminate 
$\mathcal{T}^h_u$, i.e. we consider an approximation to $\eqref{eq27}$ better
than $\eqref{eq10}$ as follows.
\begin{equation}\label{eq5.3}
\left\{
\begin{aligned}
&a_{h,\theta}(\widetilde{y}_h^{m\ast},w_h^m)=l_{h,\theta}[f+B\widetilde{u}^*,\phi]
(w_h^m),\quad\forall w_h^m\in V_h^m,\\
&a_{h,\theta}(q_h^m,\widetilde{p}_h^{m\ast})=l_{h,\theta}[g^\prime(\widetilde{y}_h^
{m\ast}),0](q_h^m),\quad\forall q_h^m\in V_h^m,\\
&(j^\prime(\widetilde{u}^*)+B^*\widetilde{p}_h^{m*},v-\widetilde{u}^*)\geq 0,
\quad \forall v\in U_{ad}.
\end{aligned}
\right.
\end{equation}

Follow the proof of Theorem $\eqref{thm2}$, we can take $v_h=u$ 
in Step 2 and derive
\[\|u-\widetilde{u}\|_{L^2}^{2}+\|\widetilde{y}_{h}^m-P_{h}{y}\|_{L^2}^{2}
\leq C(\|p-P_hp\|_{L^2}^2+\|y-P_{h}y\|_{L^2}^{2})\]
in Step 3, where $C$ depends on $\alpha,\beta.$ Consequently, we 
have
\[\|u^*-\widetilde{u}^*\|_{L^2}+
\interleave y^*-\widetilde{y}_h^{m*}\interleave_{\mathrm{DG}}+\interleave p^*-\widetilde{p}_h^{m*}\interleave_{\mathrm{DG}}\leq Ch^m.\]
For $\theta=-1$, 
\[\|u^*-\widetilde{u}^*\|_{L^2}+
\| y^*-\widetilde{y}_h^{m*}\|_{L^2}+\| p^*-\widetilde{p}_h^{m*}\|_{L^2}\leq Ch^{m+1}.\]

In practical algorithm, we rewrite the third equation in 
$\eqref{eq5.1}$ as 
\[\widetilde{u}_{ \mkern+1mu n \mkern-2mu+\mkern-2mu 1}=Pr_{U_{ad}}
(\widetilde{u}_{n}-
\rho_n(j'(\widetilde{u}_{n})+B^*\widetilde{p}_{hn}^m)),\]
and the linear convergence rate still holds.
But now we only need to store the value of $\widetilde{u}_n$ on the 
quadrature points of $\mathcal{T}^h$.

\noindent\textbf{Example 4.} Take $\Omega_u=\Omega=(0,1)^2,
B=\mathrm{Id}.$
\begin{equation*}
\begin{aligned}
&\min_{u\in L^2(\Omega_u)}\frac{1}{2}\|y-y_d\|_{L^2}^2+
\frac{1}{2}\|u-u_d\|_{L^2}^2,
&\\s.t.\ &-\Delta y=f+u,\quad y|_{\partial\Omega}=y_d|_
{\partial\Omega},\quad\int_{\Omega_u}u\mathrm{d}x\geq0.
\end{aligned}
\end{equation*}
where
\begin{equation*}
\begin{aligned}
&u_d=1-2x_1-2x_2,\quad 
p=\mathrm{sin} (\pi x_1) \mathrm{sin} (\pi x_2),\\
&y_d=0,
\quad f=4\pi^4p-u_d+p+\min\{0,\overline{u_d-p}\}.
\end{aligned}
\end{equation*}
The exact solution
\begin{equation*}
y^*=2\pi^2p+y_d,\quad u^*=u_d-p-\min\{0,\overline{u_d-p}\},
\quad p^*=p,
\end{equation*}
here $\overline{u_d-p}=\ds\frac{1}{m(\Omega)}\int_{\Omega}(
u_d-p)\mathrm{d}x.$

\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&6.305e-2&1.920e-2&5.805e-3&1.649e-3&3.857e-4\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&3.070e1&1.356e1&6.092&2.835&1.357\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&1.568&7.040e-1&3.142e-1&1.447e-1&6.887e-2\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&4.973e-2&1.231e-2&2.761e-3&6.553e-4&1.586e-4\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&2.313e1&1.015e1&4.475&2.068&9.878e-1\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&1.211&5.177e-1&2.269e-1&1.048e-1&5.005e-2\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&8.906e-1&2.015e-1&4.536e-2&1.067e-2&2.572e-3\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&5.913e-2&1.657e-2&3.882e-3&9.274e-4&2.254e-4\\
\hline
\end{tabular}
\begin{comment}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&2.25&3.38&3.87&4.09\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&0.00&2.47&2.29&2.17&2.09\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&0.00&2.46&2.71&2.41&2.16\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&2.40&3.62&4.04&4.10\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&0.00&2.56&2.28&2.17&2.09\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&0.00&2.58&2.72&2.38&2.14\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&0.00&3.00&3.87&4.27&4.19\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&0.00&2.46&3.66&4.28&4.27\\
\hline
\end{tabular}
\end{comment}
\caption{Numerical results of Example 4 for $m=1$.}
\end{table}

\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&6.806e-2&2.148e-2&5.904e-3&1.554e-3&3.986e-4\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&1.279e1&2.638&6.570e-1&1.683e-1&4.275e-2\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&9.905e-1&2.646e-1&7.396e-2&1.979e-2&5.124e-3\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&3.529e-2&3.208e-3&2.940e-4&3.013e-5&3.272e-6\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&8.851&1.971&4.732e-1&1.182e-1&2.947e-2\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&4.876e-1&1.034e-1&2.426e-2&6.007e-3&1.494e-3\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&5.601e-1&4.866e-2&4.881e-3&5.526e-4&6.292e-5\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&4.865e-2&3.630e-3&3.134e-4&3.397e-5&3.303e-6\\
\hline
\end{tabular}
\begin{comment}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&7.93&1.92&3.30&3.73\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&0.00&5.58&4.65&4.56&4.53\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&0.00&5.40&3.72&3.96&4.07\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&10.7&11.2&11.2&11.2\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&0.00&5.63&4.57&4.65&4.64\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&0.00&7.11&4.69&4.71&4.67\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&0.00&12.6&10.8&9.94&8.02\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&0.00&13.7&12.1&11.7&11.4\\
\hline
\end{tabular}
\end{comment}

\caption{Numerical results of Example 4 for $m=2$.}
\end{table}

\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&8.399e-3&5.880e-4&3.784e-5&2.685e-6&1.822e-7\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&4.442&4.009e-1&4.418e-2&4.619e-3&5.135e-4\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&2.345e-1&2.122e-2&2.290e-3&2.361e-4&2.609e-5\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&8.940e-3&4.600e-4&1.984e-5&9.752e-7&5.065e-8\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&2.914&4.125e-1&4.643e-2&5.365e-3&6.289e-4\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&1.518e-1&2.097e-2&2.353e-3&2.718e-4&3.186e-5\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&1.462e-1&8.062e-3&3.855e-4&1.918e-5&9.992e-7\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&1.022e-2&4.620e-4&1.990e-5&9.753e-7&5.065e-8\\
\hline
\end{tabular}
\begin{comment}
\end{table}
\begin{table}[H]
\centering
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&14.1&16.3&13.0&14.5\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&0.00&8.43&9.77&9.76&9.16\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&0.00&8.12&9.94&9.87&9.19\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&18.5&25.0&22.0&20.1\\
\cline{2-7}
&$\interleave y-\widetilde{y}_h^m\interleave_{\mathrm{DG}}$&0.00&8.15&10.7&9.47&8.93\\
\cline{2-7}
&$\interleave p-\widetilde{p}_h^m\interleave_{\mathrm{DG}}$&0.00&8.07&10.8&9.49&8.94\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&0.00&17.5&22.0&20.4&19.0\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&0.00&22.0&25.0&21.2&20.1\\
\hline
\end{tabular}
\end{comment}
\caption{Numerical results of Example 4 for $m=3$.}
\end{table}

==> numerical_ex.tex <==
\section{Numerical Results}
It should be noted that the approximate system $\eqref{eq10}$ 
can not be solved directly.
So we will first introduce a projected gradient descent 
method to solve $\eqref{eq10}$ iteratively in Section 5.1. In 
Section 5.2, we provide some numerical examples to validate 
the derivation in the previous sections, including a priori and a 
posteriori error estimates. In the case that the control variable has 
a smooth data, we can build another approximation to $\eqref{eq27}$
without $\mathcal{T}^h_u$, which 
means that we do not discretize the control variable. 
The proposed approximation serves to significantly improve 
computational efficiency and offers the advantage of reduced 
memory consumption.

\subsection{Practical Algorithm}
Take $u_{h0}\in U_{adh}$ as an  
initial guess to $u_h^*$ , we can then obtain a sequence \{($u_{hn},y_
{hn}^m,p_{hn}^m)\}_{n=0} ^\infty$ by the following algorithm.
\begin{equation}\label{eq5.1}
\left\{
\begin{aligned}
&a_{h,\theta}(y_{hn}^{m},w_{h}^m)=l_{h,\theta}[f+Bu_{hn}
,\phi](w_{h}^m),\quad\forall w_{h}^m\in V_h^m,\\
&a_{h,\theta}(q_h^m,p_{hn}^{m})=l_{h,\theta}[g^\prime(y_{hn}^
{m}),0](q_h^m),\quad\forall q_h^m\in V_h^m,\\
&u_{h \mkern+1mu n \mkern-2mu+\mkern-2mu 1}=Pr_{U_{adh}}
(u_{hn}-\rho_n(j'(u_{hn})+B^*p_{hn}^m)),
\end{aligned}
\right.
\end{equation}
where $Pr_{U_{adh}}:U\rightarrow U_{adh}$ is the projection
 operator and $\rho_n>0,\forall n\in \mathbb{N}.$

\begin{thm}\label{thm6}
Let $(u_h^*,y_h^{m*},p_h^{m*})$ satisfy $\eqref{eq10}$, $\{(u_{hn},
y_{hn}^m,p_{hn}^m)\}_{n=0}^\infty$ be the sequence generated by 
$\eqref{eq5.1}$. If Assumption $\eqref{ass1}$,$\eqref{ass2}$ 
hold, we can properly  
choose $\{\rho_n\}_{n=0}^\infty$ such that there exist constants
$0<\eta<1,\lambda=\lambda(\eta)>0,$ satisfy
\begin{equation*}
\begin{aligned}
&\|u_{hn}-u_h^*\|_{L^2}+\lambda\interleave y_{hn}
^m-y_h^{m*}\interleave_{\mathrm{DG}}+\lambda\interleave p_{n}^m-p_h^{m*}\interleave_{\mathrm{DG}}\\
\leq& \eta^n(\|u_{h0}-u_h^*\|_{L^2}+\lambda\interleave y_{h0}^m-y_h^{m*}\interleave_{\mathrm{DG}}+\lambda\interleave
 p_{h0}^m-p_h^{m*}\interleave_{\mathrm{DG}}).
\end{aligned}
\end{equation*}
In fact, we can show that $(u_{hn},y_{hn}^m,p_
{hn}^m)$ converges to $(u_{h}^*,y_{h}^{m*},p_{h}^{m*})$ linearly. 
\end{thm}

\begin{proof}
From now on, we omit the superscript $*$. We have
\begin{equation*}
\begin{aligned}
\|u_{h\mkern+1mu n\mkern-2mu+\mkern-2mu 1}-u_h\|_{L^2}^2=
&\|Pr_{U_{adh}}(u_{hn}-\rho_n(j'(u_{hn})+B^*p_{hn}^m))\\
&-Pr_{U_{adh}}(u_{h}-\rho_n(j'(
u_{h})+B^*p_{h}^m))\|_{L^2}^2\\
\leq&\|u_{hn}-u_{h}-\rho_n(j'(u_{hn})-j'(
u_{h})+B^*p_{hn}^m-B^*p_{h}^m)\|_{L^2}^2\\
=&\|u_{hn}-u_{h}\|_{L^2}^2+\rho_n^2\|j'(u_{hn})-j'(
u_{h})+B^*p_{hn}^m-B^*p_{h}^m\|_{L^2}^2\\
&-2\rho_n(u_{hn}-u_h,j'(u_{hn})-j'(u_h)+B^*p_{hn}^m-B^*p_h^m)\\
\leq&(1-2\alpha\rho_n+C\rho_n^2)\|u_{hn}-u_{h}\|_{L^2}^2+
C\rho_n^2\|p_{hn}^m-p_h^m\|_{L^2}^2\\
&-2\rho_n(u_{hn}-u_h,B^*p_{hn}^m-B^*p_h^m).
\end{aligned}
\end{equation*} 

From $\eqref{eq10},\eqref{eq5.1}$ we have
\begin{equation}\label{eq5.2}
\begin{aligned}
&a_{h,\theta}(y_{hn}^m-y_h^m,w_h^m)=(B(u_{hn}-u_h),w_h^m),\quad\forall w_h^m
\in V_h^m,\\
&a_{h,\theta}(q_h^m,p_{hn}^m-p_h^m)=(g^\p(y_{hn}^m)-g^\p(y_h^m),q_h^m),\quad
\forall q_h^m\in V_h^m.
\end{aligned}
\end{equation}
Let $w_h^m=p_{hn}^m-p_h^m,q_{hn}^m=y_{hn}^m-y_h^m.$ Then
\begin{equation*}
\begin{aligned}
&(u_{hn}-u_h,B^*p_{hn}^m-B^*p_h^m)=(B(u_{hn}-u_h),p_{hn}^m-
p_h^m)\\
=&(g^\p(y_{hn}^m))-g^\p(y_h^m),y_{hn}^m-y_h^m)\geq
\beta\|y_{hn}^m-y_h^m\|_{L^2}^2\geq0.
\end{aligned}
\end{equation*}
Let $w_h^m=y_{hn}^m-y_h^m,q_{hn}^m=p_{hn}^m-p_h^m.$ By the 
stability of $a_{h,\theta}$ on $(V_h^m,\interleave\cdot\interleave
_{\mathrm{DG}})$ and $\eqref{eqb}$, we know that
\[\interleave y_{hn}^m-y_h^m\interleave_{\mathrm{DG}}\leq C
\|u_{hn}-u_h\|_{L^2},
\quad\interleave p_{hn}^m-p_h^m\interleave _{\mathrm{DG}}\leq C
\|y_{hn}^m-y_h^m\|_{L^2}.\]

Consequently,
\[\|u_{h \mkern+1mu n \mkern-2mu+\mkern-2mu 1}-u_h\|_{L^2}^2
\leq(1-2\alpha\rho_n+C\rho_n^2)\|u_{hn}-u_h\|_{L^2}^2\leq
\delta^2\|u_{hn}-u_h\|_{L^2}^2,\]
where $\rho_n$ satisfies $0\leq1-2\alpha\rho_n+C\rho
_n^2\leq\delta^2<1,\forall n\in\mathbb{N}.$ 
Choose $C'$ such that
\[\interleave y_{h \mkern+1mu n \mkern-2mu+\mkern-2mu 1}^m-y_h^m\interleave_{\mathrm{DG}}+\interleave p_{h \mkern
+1mu n \mkern-2mu+\mkern-2mu 1}^m-p_h
^m\interleave_{\mathrm{DG}}\leq C'\|u_{h \mkern+1mu n \mkern
-2mu+\mkern-2mu 1}-u_h\|_{L^2},\]
and $\lambda=(1-\delta)/(2C'\delta)$. It can be verified that
\begin{equation*}
\begin{aligned}
&\|u_{h \mkern+1mu n \mkern-2mu+\mkern-2mu 1}-u_h\|_{L^2}
+\lambda\interleave y_{h \mkern+1mu n \mkern-2mu+\mkern-2mu 1}^m-y_h^m\interleave_{\mathrm{DG}}+\lambda\interleave p_{h 
\mkern+1mu n \mkern-2mu+\mkern-2mu 1}^m-p_h
^m\interleave_{\mathrm{DG}}\\
\leq& \frac{\delta+1}{2}(\|u_{hn}-u_h\|_{L^2}+\lambda\interleave y_{hn}^m-y_h^m\interleave_{\mathrm{DG}}+\lambda
\interleave p_{hn}^m-p_h^m\interleave_{\mathrm{DG}}),
\end{aligned}
\end{equation*}
which means the linear convergence rate. To complete the proof, 
we only need to take $\eta=(\delta+1)/2$.
\end{proof}

%For simplicity,  we introduce two notations
%$$[\ \cdot\ ]_{\mathrm{DG}}:=\|u^*-u_h^*\|_{L^2}
%\interleave y^*-y_h^{m*}\interleave_{\mathrm{DG}}+\interleave p^*-p_h^{m*}\interleave_{\mathrm{DG}},$$
%$$[\ \cdot\ ]_{L^2}:=\|u^*-u_h^*\|_{L^2}+
%\| y^*-y_h^{m*}\|_{L^2}+\| p^*-p_h^{m*}\|_{L^2}.$$

\subsection{Numerical Examples}
\mbox{}\\
\noindent\textbf{Examples for Convergence Order.}
We will use some examples to verify the convergance order 
proved in Theorem $\eqref{thm2}$ and Lemma $\eqref{lem2}.$

\noindent\textbf{Example 1.} Take $\Omega_u=\Omega=(0,1)^2,
B=\mathrm{Id}.$
\begin{equation*}
\begin{aligned}
&\min_{u\in L^2(\Omega_u)}\frac{1}{2}\|y-y_d\|_
{L^2}^2+\frac{1}{2}\|u-u_d\|_{L^2}^2,
&\\s.t.\ &-\Delta y=f+u,\quad y|_{\partial\Omega}=y_d|_
{\partial\Omega},\\
& u\geq 0,\quad \mathrm{a.e.\ in}\ \Omega_u.
\end{aligned}
\end{equation*}
where
\begin{equation*}
\begin{aligned}
&y_d=0,\quad u_d=1-\mathrm{sin}\frac{\pi x_1}{2}-\mathrm{sin}
\frac{\pi x_2}{2},\\
&p=\mathrm{sin} (\pi x_1) \mathrm{sin} (\pi x_2),\quad f=4\pi^4
p-\mathrm{max}\{u_d-p,0\}.
\end{aligned}
\end{equation*}
The exact solution
\begin{equation*}
y^*=2\pi^2p+y_d,\quad u^*=\mathrm{max}\{u_d-p,0\},\quad 
p^*=p.
\end{equation*}
\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&7.590e-2&3.979e-2&1.948e-2&9.683e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&3.435e1&1.390e1&6.065&2.791\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&2.367&9.616e-1&3.552e-1&1.471e-1\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&7.663e-2&3.948e-2&1.941e-2&9.675e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&3.516e1&1.372e1&6.009&2.771\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&2.411&9.357e-1&3.437e-1&1.446e-1\\
\cline{2-7}
&\multirow{3}{*}{$4h^2\ \, $}&$\|u-u_h\|_{L^2}$&7.663e-2&2.470e-2&6.552e-3&1.409e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&4.908&1.640&4.240e-1&9.923e-2\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&3.713e-1&1.507e-1&4.119e-2&9.616e-3\\
\hline
\end{tabular}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&0.00&1.91&2.04&2.01\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&0.00&2.47&2.29&2.17\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&0.00&2.46&2.71&2.42\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&0.00&1.94&2.03&2.01\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&0.00&2.56&2.28&2.17\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&0.00&2.58&2.72&2.38\\
\cline{2-7}
&\multirow{3}{*}{$4h^2\ \, $}&$\|u-u_h\|_{L^2}$&0.00&3.10&3.77&4.65\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&0.00&3.04&3.87&4.27\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&0.00&2.46&3.66&4.28\\
\hline
\end{tabular}
\caption*{\textbf{Table 1.1 Numerical results of Example 1 for $m=1$.}}
\end{table}
\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&6.442e-2&1.919e-2&4.844e-3&1.218e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&1.295e1&2.321&4.987e-1&1.092e-1\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&8.028e-1&1.487e-1&4.002e-2&1.010e-2\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&6.390e-2&1.919e-2&4.859e-3&1.217e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&1.428e1&2.534&5.550e-1&1.193e-1\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&9.602e-1&1.350e-1&2.878e-2&6.104e-3\\
\cline{2-7}
&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.390e-2&9.722e-3&1.236e-3&1.571e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&1.610&1.274e-1&1.175e-2&1.150e-3\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&1.444e-1&1.051e-2&8.720e-4&7.456e-5\\
\hline
\end{tabular}
\end{table}
\begin{table}[H]
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&0.00&3.36&3.96&3.98\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&0.00&5.58&4.65&4.57\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&0.00&5.40&3.72&3.96\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&0.00&3.33&3.95&3.99\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&0.00&5.64&4.57&4.65\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&0.00&7.11&4.69&4.71\\
\cline{2-7}
&\multirow{3}{*}{$4h^2\ \, $}&$\|u-u_h\|_{L^2}$&0.00&6.57&7.87&7.87\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&0.00&12.6&10.8&10.2\\
\cline{3-7}
	&&$\|p-p_h^m\|_{{L^2}}$&0.00&13.7&12.1&11.7\\
\hline
\end{tabular}
\caption*{\textbf{Table 1.2 Numerical results of Example 1 for $m=2$.}}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.670e-2&9.665e-3&1.217e-3&1.524e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&3.854&4.574e-1&4.678e-2&4.791e-3\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&1.942e-1&2.392e-2&2.405e-3&2.437e-4\\
\hline
\multirow{3}{*}{-1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.624e-2&9.664e-3&1.217e-3&1.523e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&3.835&4.707e-1&4.382e-2&4.625e-3\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&1.944e-1&2.408e-2&2.224e-3&2.344e-4\\
\hline
\end{tabular}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&0.00&6.90&7.94&7.99\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&0.00&8.43&9.78&9.76\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&0.00&8.12&9.95&9.87\\
\hline
\multirow{3}{*}{-1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&0.00&6.85&7.94&7.99\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&0.00&8.15&10.7&9.47\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&0.00&8.07&10.8&9.49\\
\hline
\end{tabular}
\caption*{\textbf{Table 1.3 Numerical results of Example 1 for $m=3$.}}
\end{table}
Recall that $R_h$ is the recovery operator defined in $\eqref{recover}$. 
We compute the error and convergence order of $\|u^*-R_hu_h^*
\|_{L^2}.$ 
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32&1/64&1/128\\
\hline
\multirow{2}{*}{-1}&\multirow{2}{*}{$h$}&\multirow{2}{*}{$\|u-R_hu_h\|_{L^2}$}&8.780e-2&3.587e-2&1.291e-2&4.160e-3&1.406e-3&4.832e-4\\
\cline{4-9}
&&&0.00&2.45&2.79&3.10&2.96&2.91\\
\hline
\end{tabular}
\caption*{\textbf{Table 1.4 Numerical results of Example 1 for $m=1$.}}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32&1/64&1/128\\
\hline
\multirow{2}{*}{1}&\multirow{2}{*}{$h$}&\multirow{2}{*}{$\|u-R_hu_h\|_{L^2}$}&6.758e-2&2.624e-2&1.031e-2&3.735e-3&1.327e-3&4.691e-4\\
\cline{4-9}
&&&0.00&2.58&2.55&2.76&2.81&2.83\\
\hline
\end{tabular}
\caption*{\textbf{Table 1.5 Numerical results of Example 1 for $m=2$.}}
\end{table}

\noindent\textbf{Example 2.} Take $\Omega_u=\Omega=(0,1)^2,
B=\mathrm{Id}.$
\begin{equation*}
\begin{aligned}
&\min_{u\in L^2(\Omega_u)}\frac{1}{2}\|y-y_d\|_
{L^2}^2+\frac{1}{2}\|u-u_d\|_{L^2}^2,
&\\s.t.\ &-\nabla \cdot(A\nabla y) =f+u,\quad y|_{\partial\Omega}
=y_0|_{\partial\Omega},\\
& u\geq 0,\quad \mathrm{a.e.\ in}\ \Omega_u.
\end{aligned}
\end{equation*}
where
\begin{equation*}
\begin{aligned}
&A=\begin{bmatrix}
(x+1)^2&0\\
0&(y+1)^2
\end{bmatrix}
,\quad u_d=1-\frac23x_1-\frac23x_2,\\
&p=8x_1x_2(1-x_1)(1-x_2),\quad 
y_0=-\nabla \cdot(A\nabla p),\\
&f=-\nabla\cdot(A\nabla y_0)-\mathrm{max}\{u_d-p,0\},\quad
y_d=0.
\end{aligned}
\end{equation*}
The exact solution
\begin{equation*}
y^*=y_0,\quad u^*=\mathrm{max}\{u_d-p,0\},\quad 
p^*=p.
\end{equation*}
\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&7.393e-2&3.061e-2&1.437e-2&7.053e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&2.578e1&1.178e1&5.275&2.429\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&8.059e-1&3.668e-1&1.673e-1&7.770e-2\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&8.684e-2&3.313e-2&1.472e-2&7.090e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&2.587e1&1.188e1&5.283&2.426\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&8.876e-1&3.794e-1&1.701e-1&7.809e-2\\
\cline{2-7}
&\multirow{3}{*}{$4h^2\ \, $}&$\|u-u_h\|_{L^2}$&8.684e-2&2.290e-2&5.774e-3&1.368e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&1.164&3.607e-1&9.649e-2&2.388e-2\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&7.001e-2&1.824e-2&4.592e-3&1.050e-3\\
\hline
\end{tabular}
\caption*{\textbf{Table 2.1 Numerical results of Example 2 for $m=1$.}}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&5.679e-2&1.405e-2&3.507e-3&8.770e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&7.684&1.339&2.889e-1&6.394e-2\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&3.577e-1&6.315e-2&1.253e-2&2.647e-3\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&5.821e-2&1.406e-2&3.510e-3&8.771e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&8.314&1.458&2.925e-1&6.177e-2\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&3.993e-1&6.767e-2&1.371e-2&2.920e-3\\
\cline{2-7}
&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&5.821e-2&7.103e-3&8.848e-4&1.106e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&2.448e-1&2.695e-2&2.731e-3&2.947e-4\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&2.078e-2&1.140e-3&1.175e-4&1.493e-5\\
\hline
\end{tabular}
\caption*{\textbf{Table 2.2 Numerical results of Example 2 for $m=2$.}}
\end{table}
\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&5.511e-2&7.014e-3&8.770e-4&1.089e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&1.361&9.444e-2&8.587e-3&9.587e-4\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&1.114e-1&7.828e-3&7.156e-4&7.884e-4\\
\hline
\multirow{3}{*}{-1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&5.503e-2&7.016e-3&8.770e-4&1.096e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&1.506&1.023e-1&8.952e-3&9.667e-4\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&1.216e-1&8.484e-3&7.456e-4&8.055e-5\\
\hline
\end{tabular}
\caption*{\textbf{Table 2.3 Numerical results of Example 2 for $m=3$.}}
\end{table}

\noindent\textbf{Example 3.} Take $\Omega_u=\Omega=(0,1)^2,
B=\ds\frac{1}{2}\mathrm{Id}.$
\begin{equation*}
\begin{aligned}
&\min_{u\in L^3(\Omega_u)}\frac{1}{2}\|y-y_d\|_{L^2}^2+
\frac{1}{2}\|u-u_d\|_{L^2}^2+\frac{4}{3}\|u-u_d\|_{L^3}^3,
&\\s.t.\ &-\Delta y=f+\frac{1}{2}u,\quad y|_{\partial\Omega}=y_d|_
{\partial\Omega},\\
& 0\leq u\leq 1,\quad \mathrm{a.e.\ in}\ \Omega_u.
\end{aligned}
\end{equation*}
where
\begin{equation*}
\begin{aligned}
&u_d=\frac{3}{2}-x_1- x_2,\quad p=\mathrm{sin} (\pi x_1) \mathrm
{sin} (\pi x_2),\\
&y_d=0,\quad f=4
\pi^4p-\frac{1}{2}Pr_{[0,1]}(u_d-s(p)).
\end{aligned}
\end{equation*}
The exact solution
\begin{equation*}
y^*=2\pi^2p+y_d,\quad u^*=Pr_{[0,1]}(u_d-s(p)),\quad 
p^*=p,
\end{equation*}
where $s(p)$ is an implicit function satisfies \[s(p)+4
s(p)^2\mathrm{sgn}(s(p))=\frac{1}{2}p,\]
and $Pr_{[0,1]}(s):=\min\{\max\{s,0\},1\}.$
\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&1.109e-1&4.678e-2&1.887e-2&8.599e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&3.435e1&1.390e1&6.065&2.791\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&2.367&9.615e-1&3.552e-1&1.471e-1\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$h$}&$\|u-u_h\|_{L^2}$&1.125e-1&4.572e-2&1.847e-2&8.537e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&3.516e1&1.372e1&6.009&2.771\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&2.411&9.356e-1&3.437e-1&1.446e-1\\
\cline{2-7}
&\multirow{3}{*}{$4h^2\ \, $}&$\|u-u_h\|_{L^2}$&1.125e-1&3.463e-2&8.783e-3&2.061e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&4.907&1.640&4.239e-1&9.919e-2\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&3.713e-1&1.507e-1&4.118e-2&9.614e-3\\
\hline
\end{tabular}
\caption*{\textbf{Table 3.1 Numerical results of Example 3 for $m=1$.}}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&7.162e-2&1.697e-2&4.498e-3&1.135e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&1.295e1&2.320&4.985e-1&1.092e-1\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&8.027e-1&1.486e-1&4.001e-2&1.010e-2\\
\hline
\multirow{6}{*}{-1}&\multirow{3}{*}{$4h^2$}&$\|u-u_h\|_{L^2}$&7.510e-2&1.675e-2&4.715e-3&1.044e-3\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&1.428e1&2.534&5.550e-1&1.193e-1\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&9.600e-1&1.350e-1&2.878e-2&6.104e-3\\
\cline{2-7}
&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&7.510e-2&8.558e-3&1.058e-3&1.348e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{{L^2}}$&1.610&1.274e-1&1.174e-2&1.180e-3\\
\cline{3-7}
&&$\|p-p_h^m\|_{{L^2}}$&1.444e-1&1.051e-2&8.718e-4&7.454e-5\\
\hline
\end{tabular}
\caption*{\textbf{Table 3.2 Numerical results of Example 3 for $m=2$.}}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&$h_u$&norm&1/4&1/8&1/16&1/32\\
\hline
\multirow{3}{*}{1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.697e-2&8.333e-3&1.044e-3&1.305e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&3.854&4.572e-1&4.678e-2&4.791e-3\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&1.942e-1&2.391e-2&2.405e-3&2.437e-4\\
\hline
\multirow{3}{*}{-1}&\multirow{3}{*}{$16h^3$}&$\|u-u_h\|_{L^2}$&6.713e-2&8.347e-3&1.044e-3&1.305e-4\\
\cline{3-7}
&&$\|y-y_h^m\|_{\mathrm{DG}}$&3.835&4.707e-1&4.383e-2&4.625e-3\\
\cline{3-7}
&&$\|p-p_h^m\|_{\mathrm{DG}}$&1.944e-1&2.407e-2&2.224e-3&2.344e-4\\
\hline
\end{tabular}
\caption*{\textbf{Table 3.3 Numerical results of Example 3 for $m=3$.}}
\end{table}

\noindent\textbf{Smooth Example.}
Notice that in Theorem $\eqref{thm2}$ and Lemma $\eqref{lem2}$, the order 
of $h_u$ is rather small compared to $h$, which leads to more refinement on 
$\mathcal{T}^h_u$. In order to optimize computional efficiency and minimize
memory cost, we can calculate $u$ without discretization and eliminate 
$\mathcal{T}^h_u$, i.e. we consider an approximation to $\eqref{eq27}$ better
than $\eqref{eq10}$ as follows.
\begin{equation}\label{eq5.3}
\left\{
\begin{aligned}
&a_{h,\theta}(\widetilde{y}_h^{m\ast},w_h^m)=l_{h,\theta}[f+B\widetilde{u}^*,\phi]
(w_h^m),\quad\forall w_h^m\in V_h^m,\\
&a_{h,\theta}(q_h^m,\widetilde{p}_h^{m\ast})=l_{h,\theta}[g^\prime(\widetilde{y}_h^
{m\ast}),0](q_h^m),\quad\forall q_h^m\in V_h^m,\\
&(j^\prime(\widetilde{u}^*)+B^*\widetilde{p}_h^{m*},v-\widetilde{u}^*)\geq 0,
\quad \forall v\in U_{ad}.
\end{aligned}
\right.
\end{equation}

Follow the proof of Theorem $\eqref{thm2}$, we can take $v_h=u$ 
in Step 2 and derive
\[\|u-\widetilde{u}\|_{L^2}^{2}+\|\widetilde{y}_{h}^m-P_{h}{y}\|_{L^2}^{2}
\leq C(\|p-P_hp\|_{L^2}^2+\|y-P_{h}y\|_{L^2}^{2})\]
in Step 3, where $C$ depends on $\alpha,\beta.$ Consequently, we 
have
\[\|u^*-\widetilde{u}^*\|_{L^2}+
\interleave y^*-\widetilde{y}_h^{m*}\interleave_{\mathrm{DG}}+\interleave p^*-\widetilde{p}_h^{m*}\interleave_{\mathrm{DG}}\leq Ch^m.\]
For $\theta=-1$, 
\[\|u^*-\widetilde{u}^*\|_{L^2}+
\| y^*-\widetilde{y}_h^{m*}\|_{L^2}+\| p^*-\widetilde{p}_h^{m*}\|_{L^2}\leq Ch^{m+1}.\]

In practical algorithm, we rewrite the third equation in 
$\eqref{eq5.1}$ as 
\[\widetilde{u}_{ \mkern+1mu n \mkern-2mu+\mkern-2mu 1}=Pr_{U_{ad}}
(\widetilde{u}_{n}-
\rho_n(j'(\widetilde{u}_{n})+B^*\widetilde{p}_{hn}^m)),\]
and the linear convergence rate still holds.
But now we only need to store the value of $\widetilde{u}_n$ on the 
quadrature points of $\mathcal{T}^h$.

\noindent\textbf{Example 4.} Take $\Omega_u=\Omega=(0,1)^2,
B=\mathrm{Id}.$
\begin{equation*}
\begin{aligned}
&\min_{u\in L^2(\Omega_u)}\frac{1}{2}\|y-y_d\|_{L^2}^2+
\frac{1}{2}\|u-u_d\|_{L^2}^2,
&\\s.t.\ &-\Delta y=f+u,\quad y|_{\partial\Omega}=y_d|_
{\partial\Omega},\quad\int_{\Omega_u}u\mathrm{d}x\geq0.
\end{aligned}
\end{equation*}
where
\begin{equation*}
\begin{aligned}
&u_d=1-2x_1-2x_2,\quad 
p=\mathrm{sin} (\pi x_1) \mathrm{sin} (\pi x_2),\\
&y_d=0,
\quad f=4\pi^4p-u_d+p+\min\{0,\overline{u_d-p}\}.
\end{aligned}
\end{equation*}
The exact solution
\begin{equation*}
y^*=2\pi^2p+y_d,\quad u^*=u_d-p-\min\{0,\overline{u_d-p}\},
\quad p^*=p,
\end{equation*}
here $\overline{u_d-p}=\ds\frac{1}{m(\Omega)}\int_{\Omega}(
u_d-p)\mathrm{d}x.$

\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&2.178e-1&9.681e-2&2.866e-2&7.407e-3&1.809e-3\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&3.434e1&1.390e1&6.064&2.791&1.333\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&2.367&9.612e-1&3.551e-1&1.471e-1&6.818e-2\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&2.217e-1&9.223e-2&2.551e-2&6.312e-3&1.541e-3\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&3.515e1&1.372e1&6.008&2.771&1.327\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&2.411&9.354e-1&3.436e-1&1.446e-1&6.770e-2\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&4.906&1.637&4.233e-1&9.906e-2&2.363e-2\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&3.712e-1&1.507e-1&4.116e-2&9.607e-3&2.248e-3\\
\hline
\end{tabular}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&2.25&3.38&3.87&4.09\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&0.00&2.47&2.29&2.17&2.09\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&0.00&2.46&2.71&2.41&2.16\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&2.40&3.62&4.04&4.10\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&0.00&2.56&2.28&2.17&2.09\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&0.00&2.58&2.72&2.38&2.14\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&0.00&3.00&3.87&4.27&4.19\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&0.00&2.46&3.66&4.28&4.27\\
\hline
\end{tabular}
\caption*{\textbf{Table 4.1 Numerical results of Example 4 for $m=1$.}}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&7.380e-2&9.310e-3&4.860e-3&1.471e-3&3.939e-4\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&1.295e1&2.320&4.984e-1&1.092e-1&2.413e-2\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&8.025e-1&1.486e-1&3.999e-2&1.010e-2&2.483e-3\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&9.477e-2&8.878e-3&7.946e-4&7.066e-5&6.332e-6\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&1.427e1&2.534&5.550e-1&1.193e-1&2.570e-2\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&9.598e-1&1.350e-1&2.878e-2&6.104e-3&1.306e-3\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&1.608&1.272e-1&1.173e-2&1.180e-3&1.471e-4\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&1.443e-1&1.050e-2&8.711e-4&7.451e-5&6.511e-6\\
\hline
\end{tabular}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&7.93&1.92&3.30&3.73\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&0.00&5.58&4.65&4.56&4.53\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&0.00&5.40&3.72&3.96&4.07\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&10.7&11.2&11.2&11.2\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&0.00&5.63&4.57&4.65&4.64\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&0.00&7.11&4.69&4.71&4.67\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&0.00&12.6&10.8&9.94&8.02\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&0.00&13.7&12.1&11.7&11.4\\
\hline
\end{tabular}
\caption*{\textbf{Table 4.2 Numerical results of Example 4 for $m=2$.}}
\end{table}
\begin{table}[H]
\centering
\renewcommand\arraystretch{1.0}
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&8.381e-3&5.960e-4&3.667e-5&2.826e-6&1.952e-7\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&3.854&4.572e-1&4.678e-2&4.791e-3&5.228e-4\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&1.942e-1&2.391e-2&2.405e-3&2.437e-4&2.651e-5\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&1.099e-2&5.937e-4&2.379e-5&1.128e-6&5.623e-8\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&3.835&4.707e-1&4.382e-2&4.625e-3&5.177e-4\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&1.944e-1&2.407e-2&2.224e-3&2.344e-4&2.623e-5\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&1.761e-1&1.009e-2&4.577e-4&2.247e-5&1.187e-6\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&1.313e-2&5.970e-4&2.387e-5&1.128e-6&5.623e-8\\
\hline
\end{tabular}
\end{table}
\begin{table}[H]
\centering
\begin{tabular}{l|l|l|l|l|l|l}
\hline
$\theta$&norm&1/4&1/8&1/16&1/32&1/64\\
\hline
\multirow{3}{*}{1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&14.1&16.3&13.0&14.5\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&0.00&8.43&9.77&9.76&9.16\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&0.00&8.12&9.94&9.87&9.19\\
\hline
\multirow{5}{*}{-1}&$\|u-\widetilde{u}\|_{L^2}$&0.00&18.5&25.0&22.0&20.1\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{\mathrm{DG}}$&0.00&8.15&10.7&9.47&8.93\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{\mathrm{DG}}$&0.00&8.07&10.8&9.49&8.94\\
\cline{2-7}
&$\|y-\widetilde{y}_h^m\|_{L^2}$&0.00&17.5&22.0&20.4&19.0\\
\cline{2-7}
&$\|p-\widetilde{p}_h^m\|_{L^2}$&0.00&22.0&25.0&21.2&20.1\\
\hline
\end{tabular}
\caption*{\textbf{Table 4.3 Numerical results of Example 4 for $m=3$.}}
\end{table}
